Picard and Chazy solutions to the Painleve' VI equation

I study the solutions of a particular family of Painlev\'e VI equations with the parameters $\beta=\gamma=0, \delta=1/2$ and $2\alpha=(2\mu-1)^2$, for $2\mu\in\interi$. I show that the case of half-integer $\mu$ is integrable and that the solutions are of two types: the so-called Picard solutions and the so-called Chazy solutions. I give explicit formulae for them and completely determine their asymptotic behaviour near the singular points $0,1,\infty$ and their nonlinear monodromy. I study the structure of analytic continuation of the solutions to the PVI$\mu$ equation for any $\mu$ such that $2\mu\in\interi$. As an application, I classify all the algebraic solutions. For $\mu$ half-integer, I show that they are in one to one correspondence with regular polygons or star-polygons in the plane. For $\mu$ integer, I show that all algebraic solutions belong to a one-parameter family of rational solutions.

==> nuovisimboli.tex <==
%  aggiornato al 5/3/94
%
\catcode`@=11
%
%---------------------------- \lsim \gsim ----------------------------------
%
%    Simboli di minore o circa uguale, maggiore o circa uguale.
%
\def\lsim{\mathchoice
  {\mathrel{\lower.8ex\hbox{$\displaystyle\buildrel<\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\textstyle\buildrel<\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\scriptstyle\buildrel<\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\scriptscriptstyle\buildrel<\over\sim$}}} }
\def\gsim{\mathchoice
  {\mathrel{\lower.8ex\hbox{$\displaystyle\buildrel>\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\textstyle\buildrel>\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\scriptstyle\buildrel>\over\sim$}}}
  {\mathrel{\lower.8ex\hbox{$\scriptscriptstyle\buildrel>\over\sim$}}} }
%
%
%---------------------------  \quadratello ---------------------------------
%
%
\def\quad@rato#1#2{{\vcenter{\vbox{
        \hrule height#2pt
        \hbox{\vrule width#2pt height#1pt \kern#1pt \vrule width#2pt}
        \hrule height#2pt} }}}
\def\quadratello{\mathchoice
\quad@rato5{.5}\quad@rato5{.5}\quad@rato{3.5}{.35}\quad@rato{2.5}{.25} }
%
%------------------------ caratteri grassetto speciali -----------
%
\font\s@a=cmss10\font\s@b=cmss8
\def\reali{{\mathchoice
 {\hbox{\s@a l\kern-.5mm R}}
 {\hbox{\s@a l\kern-.5mm R}}
 {\hbox{\s@b l\kern-.4mm R}}
 {\hbox{\s@b l\kern-.4mm R}}  }}
\def\naturali{{\mathchoice
 {\hbox{\s@a l\kern-.5mm N}}
 {\hbox{\s@a l\kern-.5mm N}}
 {\hbox{\s@b l\kern-.4mm N}}
 {\hbox{\s@b l\kern-.4mm N}}  }}
\def\interi{{\mathchoice
 {\hbox{\s@a Z\kern-1.5mm Z}}
 {\hbox{\s@a Z\kern-1.5mm Z}}
 {\hbox{{\s@b Z\kern-1.2mm Z}}}
 {\hbox{{\s@b Z\kern-1.2mm Z}}}  }}
\def\complessi{{\mathchoice
 {\hbox{\s@a C\kern-1.4mm\raise.2mm\hbox{\s@b l}\kern.8mm}}
 {\hbox{\s@a C\kern-1.4mm\raise.2mm\hbox{\s@b l}\kern.8mm}}
 {\hbox{\s@b C\kern-1.1mm\raise.13mm\hbox{\s@b l}\kern.5mm}}
 {\hbox{\s@b C\kern-1.1mm\raise.13mm\hbox{\s@b l}\kern.5mm}} }}
\def\toro{{\mathchoice
 {\hbox{\s@a T\kern-1.9mm T}}
 {\hbox{\s@a T\kern-1.9mm T}}
 {\hbox{\s@b T\kern-1.4mm T}}
 {\hbox{\s@b T\kern-1.4mm T}}  }}
\def\unity{{\hbox{\s@a 1\kern-.8mm l}}}
%
% gli stessi, per le note in \eightpoint
%
\def\footreali{\hbox{\s@b l\kern-.4mm R}}
\def\footnaturali{\hbox{\s@b l\kern-.4mm N}}
\def\footinteri{\hbox{{\s@b Z\kern-1.2mm Z}}}
\def\footcomplessi{\hbox{\s@b C\kern-1.1mm\raise.13mm\hbox{\s@b l}\kern.5mm}}
\def\foottoro{\hbox{\s@b T\kern-1.4mm T}}

%
%------------------------- bold math. it. --------------------------
%
\font\bold@mit=cmmib10
\def\setbmit{\textfont1=\bold@mit}
\def\bmit#1{\hbox{\textfont1=\bold@mit$#1$}}
%
%-----------------------------------------------------------------
\catcode`@=12

